Nonlinear electronic density response of the ferromagnetic uniform electron gas at warm dense matter conditions

In a recent Letter [T.~Dornheim \emph{et al.}, Phys.~Rev.~Lett.~\textbf{125}, 085001 (2020)], we have presented the first \emph{ab initio} results for the nonlinear density response of electrons in the warm dense matter regime. In the present work, we extend these efforts by carrying out extensive new path integral Monte Carlo (PIMC) simulations of a \emph{ferromagnetic} electron gas that is subject to an external harmonic perturbation. This allows us to unambiguously quantify the impact of spin-effects on the nonlinear density response of the warm dense electron gas. In addition to their utility for the description of warm dense matter in an external magnetic field, our results further advance our current understanding of the uniform electron gas as a fundamental model system, which is important in its own right.

==> old_bibitems.tex <==
\begin{thebibliography}{10}


\bibitem{quantum_theory} G.~Giuliani and G.~Vignale, Quantum Theory of the Electron Liquid, Cambridge University Press (2008)


\bibitem{loos} P.-F.~Loos and P.M.W.~Gill, The uniform electron gas, \href{http://onlinelibrary.wiley.com/doi/10.1002/wcms.1257/abstract}{ \textit{Comput.~Mol.~Sci.}~\textbf{6}, 410-429 } (2016)


\bibitem{review} T.~Dornheim, S.~Groth, and M.~Bonitz, The uniform electron gas at warm dense matter conditions,
\href{https://www.sciencedirect.com/science/article/abs/pii/S0370157318300516}{\textit{Phys.~Reports}~\textbf{744}, 1--86} (2018)

\bibitem{Dandrea_PRB}
R.G. Dandrea, N.W. Ashcroft, A.E. Carlsson, Electron liquid at any degeneracy, Phys. Rev. B {\bf 34}, 2097 (1986).




\bibitem{pines} D.~Bohm and D.~Pines, A Collective Description of Electron Interactions: II. Collective vs Individual Particle Aspects of the Interactions, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.85.338}{\textit{Phys.~Rev.}~\textbf{85}, 338} (1952)

\bibitem{bcs} J.~Bardeen, L.N.~Cooper, and J.R.~Schrieffer, Theory of superconductivity \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.108.1175}{\textit{Phys.~Rev.}~\textbf{108}, 1175} (1957)
















% Wigner crystallization

\bibitem{wigner} E.~Wigner, On the interaction of electrons in metals, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.46.1002}{\textit{Phys.~Rev.}~\textbf{46}, 1002} (1934)




\bibitem{drummond_wigner} N.D.~Drummond, Z.~Radnai, J.R.~Trail, M.D.~Towler, and R.J.~Needs, Diffusion quantum Monte Carlo study of three-dimensional Wigner crystals, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.69.085116}{\textit{Phys.~Rev.~B} \textbf{69}, 085116} (2004)









\bibitem{vwn} S.H.~Vosko, L.~Wilk, and M.~Nusair, Accurate Spin-Dependent Electron Liquid Correlation Energies for Local Spin Density Calculations: A Critical Analysis, \href{ http://www.nrcresearchpress.com/doi/abs/10.1139/p80-159}{ \textit{Can.~J.~Phys.}~\textbf{58}, 1200} (1980)


\bibitem{perdew} J.P.~Perdew and A.~Zunger, Self-interaction correction to density-functional approximations for many-electron systems, \href{ http://link.aps.org/doi/10.1103/PhysRevB.23.5048 }{ \textit{Phys.~Rev.~B} \textbf{23}, 5048 } (1981)

\bibitem{perdew_wang} J.P.~Perdew and Y.~Wang, Pair-distribution function and its coupling-constant average for the spin-polarized electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.46.12947}{\textit{Phys.~Rev.~B} \textbf{46}, 12947} (1992)

\bibitem{gori-giorgi1} P.~Gori-Giorgi, F.~Sacchetti, and G.B.~Bachelet, Analytic static structure factors and pair-correlation functions for the unpolarized homogeneous electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.61.7353}{\textit{Phys.~Rev.~B} \textbf{61}, 7353} (2000)

\bibitem{gori-giorgi2} P.~Gori-Giorgi and J.P.~Perdew, Pair distribution function of the spin-polarized electron gas: A first-principles analytic model for all uniform densities, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.66.165118}{\textit{Phys.~Rev.~B} \textbf{66}, 165118} (2002)














\bibitem{gs2} D.M.~Ceperley and B.J.~Alder, Ground State of the Electron Gas by a Stochastic Method, \href{ http://link.aps.org/doi/10.1103/PhysRevLett.45.566}{ \textit{Phys. Rev. Lett.} \textbf{45}, 566} (1980)





\bibitem{moroni2} S.~Moroni, D.M.~Ceperley, and G.~Senatore, Static Response and Local Field Factor of the Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevLett.75.689}{\textit{Phys.~Rev.~Lett.}~\textbf{75}, 689} (1995)


\bibitem{spink} G.G.~Spink, R.J.~Needs, and N.D.~Drummond, Quantum Monte Carlo study of the three-dimensional spin-polarized homogeneous electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.88.085121}{\textit{Phys.~Rev.~B}~\textbf{88}, 085121} (2013)

\bibitem{ortiz1} G.~Ortiz and P.~Ballone, Correlation energy, structure factor, radial distribution function, and momentum distribution of the spin-polarized uniform electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.50.1391}{\textit{Phys.~Rev.~B} \textbf{50}, 1391} (1994)

\bibitem{ortiz2} G.~Ortiz, M.~Harris, and P.~Ballone, Zero Temperature Phases of the Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.82.5317}{\textit{Phys.~Rev.~Lett.}~\textbf{82}, 5317} (1999)








\bibitem{dft_review} R.O.~Jones, Density functional theory: Its origins, rise to prominence, and future, \href{ https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.87.897 }{ \textit{Rev.~Mod.~Phys.}~\textbf{87}, 897 } (2015)

\bibitem{burke_perspective} K.~Burke, Perspective on density functional theory, \href{https://aip.scitation.org/doi/10.1063/1.4704546}{\textit{J.~Chem.~Phys.}~\textbf{136}, 150901} (2012)




























% Giant planet interiors

\bibitem{militzer1} J.~Vorberger, I.~Tamblyn, B.~Militzer, and S.A.~Bonev, Hydrogen-helium mixtures in the interiors of giant planets, \href{ https://journals.aps.org/prb/abstract/10.1103/PhysRevB.75.024206 }{
\textit{Phys.~Rev.~B} \textbf{75}, 024206} (2007)



% ### Brown dwarfs
\bibitem{saumon1} D.~Saumon, W.B.~Hubbard, G.~Chabrier, and H.M.~van~Horn, The role of the
molecular-metallic transition of hydrogen in the evolution of Jupiter, Saturn, and
brown dwarfs, \href{http://adsabs.harvard.edu/full/1992ApJ...391..827S}{ \textit{Astrophys.~J.}~\textbf{391}, 827-831} (1992)


\bibitem{becker} A.~Becker, W.~Lorenzen, J.J.~Fortney, N.~Nettelmann, M.~Sch\"ottler, and R.~Redmer, Ab initio equations of state for
hydrogen (H-REOS.3) and helium (He-REOS.3) and their
implications for the interior of brown dwarfs, \href{https://iopscience.iop.org/article/10.1088/0067-0049/215/2/21/meta}{ \textit{Astrophys.~J.~Suppl.~Ser.}~\textbf{215}, 21} (2014)









% Fusion and stuff, ICF

\bibitem{hu_ICF} S.X.~Hu, B.~Militzer, V.N.~Goncharov, and S.~Skupsky, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.84.224109}{\textit{Phys.~Rev.~B} \textbf{84}, 224109} (2011)







\bibitem{torben_eur} T.~Ott, H.~Thomsen, J.W.~Abraham, T.~Dornheim, and M.~Bonitz, Recent progress in the theory and simulation of strongly correlated plasmas: phase transitions, transport, quantum, and magnetic field effects, \href{https://link.springer.com/article/10.1140/epjd/e2018-80385-7}{\textit{Eur.~Phys.~J.~D} \textbf{72}, 84} (2018)









% WDM experiment overview

\bibitem{falk_wdm} K.~Falk, Experimental methods for warm dense matter research, \href{https://www.cambridge.org/core/journals/high-power-laser-science-and-engineering/article/experimental-methods-for-warm-dense-matter-research/7205AE1029BEA0061044F84875F1CEDB}{\textit{High Power Laser Sci. Eng.}~\textbf{6}, e59} (2018)














% Spectacular experimental success:

\bibitem{exp1} D.~Kraus \textit{et al.}, Nanosecond formation of diamond and lonsdaleite by shock compression of graphite, \href{https://www.nature.com/articles/ncomms10970}{\textit{Nature Comm.}~\textbf{7}, 10970} (2016)

\bibitem{exp2} D.~Kraus \textit{et al.}, Formation  of  diamonds  in  laser-compressedhydrocarbons at planetary interior conditions, \href{https://www.nature.com/articles/s41550-017-0219-9?dom=prime&src=syn}{\textit{Nature Astronomy} \textbf{1}, 606-611} (2017)

\bibitem{exp3} A.L.~Kritcher, P.~Neumayer, J.~Castor, T.~D\"oppner, R.W.~Falcone, O.L.~Landen, H.J.~Lee, R.W.~Lee, E.C.~Morse, A.~Ng, S.~Pollaine, D.~Price, and S.H.~Glenzer, Ultrafast X-ray Thomson Scattering of Shock-Compressed Matter, \href{https://science.sciencemag.org/content/322/5898/69?casa_token=gnFVMXKwtFIAAAAA:-1mC8CHI-ffNXXfE2a6glDad_Von_3xGVRUUqpa8N6aOGGGsHxQvFletxgFvbnJLATqfGQHtB1LcWA}{\textit{Science} \textbf{322}, 69-71} (2008)

\bibitem{exp4}   M.Z.~Mo, Z.~Chen, R. K. Li, M. Dunning, B. B. L. Witte, J. K. Baldwin, L. B. Fletcher, J. B. Kim,A. Ng, R. Redmer, A. H. Reid, P. Shekhar, X. Z. Shen, M. Shen, K. Sokolowski-Tinten, Y. Y.Tsui, Y. Q. Wang, Q. Zheng, X. J. Wang, and S. H. Glenzer, Heterogeneous to homogeneous melting transition visualized with ultrafast electron diffraction, \href{https://science.sciencemag.org/content/360/6396/1451.abstract?casa_token=g9WE5wjZu_QAAAAA:WqzLgiMM_HQL3Yqil8pvJ0xu6EtKgDy61EpycMKXEJXbqxeAC1WTZeOlqDe4g0Cd2oyfb0jQtk9tag}{\textit{Science} \textbf{360}, 1451-1455} (2018)








% WDM theory general book

\bibitem{wdm_book} F.~Graziani, M.P.~Desjarlais, R.~Redmer, and S.B.~Trickey (eds.), Frontiers and Challenges in Warm Dense Matter, Springer International Publishing (2014)



\bibitem{new_POP} M.~Bonitz, T.~Dornheim, Zh.A.~Moldabekov, S.~Zhang, P.~Hamann, H.~K\"ahlert, A.~Filinov, K.~Ramakrishna, and J.~Vorberger, Ab initio simulation of warm dense matter,
\href{https://doi.org/10.1063/1.5143225}{\textit{Phys. Plasmas} \textbf{27} (4), 042710} (2020)


\bibitem{kas1} J.J.~Kas and J.J.~Rehr, Finite Temperature Green’s Function Approach for Excited State and Thermodynamic Properties of Cool to Warm Dense Matter, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.176403}{\textit{Phys.~Rev.~Lett.}~\textbf{119}, 176403} (2017)


\bibitem{kas3} T.S.~Tan, J.J.~Kas, and J.J.~Rehr, Coulomb-hole and screened exchange in the electron self-energy at finite temperature, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.98.115125}{\textit{Phys.~Rev.~B}~\textbf{98}, 115125} (2018)






% semi-classical MD

\bibitem{MD1} A.~Filinov, V.~Golubnychiy, M.~Bonitz, W.~Ebeling, and J.~Dufty, Temperature-dependent quantum pair potentials and their application to dense partially ionized hydrogen plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.70.046411}{\textit{Phys.~Rev.~E} \textbf{70}, 046411} (2004)

\bibitem{MD2} W.~Ebeling, A.~Filinov, M.~Bonitz, V.~Filinov, and T.~Pohl, 
The method of effective potentials in the quantum-statistical theory of plasmas, 
%Journal of Physics A: Mathematical and General
 \href{https://iopscience.iop.org/article/10.1088/0305-4470/39/17/S01/meta}{\textit{J.~Phys. A: Math.~Gen.}~\textbf{39}, 4309-4317} (2006)

















\bibitem{dornheim_sign_problem} T.~Dornheim, Fermion sign problem in path integral Monte Carlo simulations: Quantum dots, ultracold atoms, and warm dense matter, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.100.023307}{\textit{Phys.~Rev.~E} \textbf{100}, 023307} (2019)





\bibitem{loh} E.Y.~Loh, J.E.~Gubernatis, R.T.~Scalettar, S.R.~White, D.J.~Scalapino and R.L.~Sugar, Sign problem in the numerical simulation of many-electron systems, \href{http://link.aps.org/doi/10.1103/PhysRevB.41.9301}{\textit{Phys. Rev. B} \textbf{41}, 9301-9307} (1990)


\bibitem{troyer} M.~Troyer and U.J.~Wiese, Computational Complexity and Fundamental Limitations to Fermionic Quantum Monte Carlo Simulations, \href{http://link.aps.org/doi/10.1103/PhysRevLett.94.170201}{\textit{Phys. Rev. Lett.} \textbf{94}, 170201} (2005)













\bibitem{brown_ethan} E.W.~Brown, B.K.~Clark, J.L.~DuBois, and D.M.~Ceperley, Path-Integral Monte Carlo Simulation of the Warm Dense Homogeneous Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.110.146405}{\textit{Phys.~Rev.~Lett.}~\textbf{110}, 146405} (2013)







\bibitem{schoof_prl} T.~Schoof, S.~Groth, J.~Vorberger, and M.~Bonitz, \textit{Ab Initio} Thermodynamic Results for the Degenerate Electron Gas at Finite Temperature, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.115.130402}{\textit{Phys.~Rev.~Lett.}~\textbf{115}, 130402} (2015)






\bibitem{dornheim_prl} T.~Dornheim, S.~Groth, T.~Sjostrom, F.D.~Malone, W.M.C.~Foulkes, and M.~Bonitz, \textit{Ab Initio}   Quantum Monte Carlo Simulation of the Warm Dense Electron Gas in the Thermodynamic Limit, \href{ http://link.aps.org/doi/10.1103/PhysRevLett.117.156403}{\textit{Phys.~Rev.~Lett.}~\textbf{117}, 156403} (2016)



\bibitem{groth_prl} S.~Groth, T.~Dornheim, T.~Sjostrom, F.D.~Malone, W.M.C.~Foulkes, and M.~Bonitz, \textit{Ab initio} Exchange--Correlation Free Energy of the Uniform Electron Gas at Warm Dense Matter Conditions, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.135001}{\textit{Phys.~Rev.~Lett.}~\textbf{119}, 135001} (2017)




\bibitem{malone2} F.D.~Malone, N.S.~Blunt, E.W.~Brown, D.K.K.~Lee, J.S.~Spencer, W.M.C.~Foulkes, and J.J.~Shepherd, Accurate Exchange-Correlation Energies for the Warm Dense Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.117.115701}{\textit{Phys.~Rev.~Lett.}~\textbf{117}, 115701} (2016)

\bibitem{dornheim_pop} T.~Dornheim, S.~Groth, F.D.~Malone, T. Schoof, T.~Sjostrom, W.M.C.~Foulkes, and M.~Bonitz, \textit{Ab Initio}   Quantum Monte Carlo Simulation of the Warm Dense Electron Gas, \href{ http://aip.scitation.org/doi/full/10.1063/1.4977920}{ \textit{Phys.~Plasmas}  {\bf 24}, 056303} (2017)




















\bibitem{dornheim} T.~Dornheim, S.~Groth, A.~Filinov and M.~Bonitz, Permutation blocking path integral Monte Carlo: a highly efficient approach to the simulation of strongly degenerate non-ideal fermions, \href{ http://iopscience.iop.org/1367-2630/17/7/073017 }{ \textit{New J. Phys.} \textbf{17}, 073017} (2015)

\bibitem{dornheim2} T.~Dornheim, T.~Schoof, S.~Groth, A.~Filinov, and M.~Bonitz, Permutation Blocking Path Integral Monte Carlo Approach to the Uniform Electron Gas at Finite Temperature, \href{ http://scitation.aip.org/content/aip/journal/jcp/143/20/10.1063/1.4936145 }{ \textit{ J. Chem. Phys.} \textbf{143}, 204101} (2015)



\bibitem{groth} S.~Groth, T.~Schoof, T.~Dornheim, and M.~Bonitz, \textit{Ab Initio} Quantum Monte Carlo Simulations of the Uniform Electron Gas without Fixed Nodes, \href{ http://link.aps.org/doi/10.1103/PhysRevB.93.085102 }{ \textit{Phys.~Rev.~B} \textbf{93}, 085102} (2016)


\bibitem{dornheim3} T.~Dornheim, S.~Groth, T.~Schoof, C.~Hann, and M.~Bonitz, \textit{Ab initio} quantum Monte Carlo simulations of the Uniform electron gas without fixed nodes: The unpolarized case, \href{ http://link.aps.org/doi/10.1103/PhysRevB.93.205134 }{ \textit{Phys.~Rev.~B} \textbf{93}, 205134 } (2016)



\bibitem{dornheim_cpp} T.~Dornheim, S.~Groth, and M.~Bonitz, Ab initio results for the Static Structure Factor of the Warm Dense Electron Gas, \href{https://onlinelibrary.wiley.com/doi/full/10.1002/ctpp.201700096}{\textit{Contrib.~Plasma Phys.}~\textbf{57}, 468-478} (2017)



\bibitem{blunt} N.S.~Blunt, T.W.~Rogers, J.S.~Spencer, and W.M.C.~Foulkes, Density-matrix quantum Monte Carlo method, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.89.245124}{\textit{Phys.~Rev.~B} \textbf{89}, 245124} (2014)


\bibitem{malone1} F.D.~Malone, N.S.~Blunt, J.J.~Shepherd, D.K.K.~Lee, J.S.~Spencer, and W.M.C.~Foulkes, Interaction picture density matrix quantum Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.4927434}{\textit{J.~Chem.~Phys.}~\textbf{143}, 044116} (2015)

\bibitem{malone2} F.D.~Malone, N.S.~Blunt, E.W.~Brown, D.K.K.~Lee, J.S.~Spencer, W.M.C.~Foulkes, and J.J.~Shepherd, Accurate Exchange-Correlation Energies for the Warm Dense Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.117.115701}{\textit{Phys.~Rev.~Lett.}~\textbf{117}, 115701} (2016)




\bibitem{dornheim_neu} T.~Dornheim, S.~Groth, and M.~Bonitz, Permutation Blocking Path Integral Monte Carlo Simulations of Degenerate Electrons at Finite Temperature, \href{https://onlinelibrary.wiley.com/doi/full/10.1002/ctpp.201800157}{\textit{Contrib.~Plasma Phys.}~\textbf{59}, e201800157} (2019)














\bibitem{karasiev_status} V.V.~Karasiev, S.B.~Trickey, and J.W.~Dufty, Status of free-energy representations for the homogeneous electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.195134}{\textit{Phys.~Rev.~B} \textbf{99}, 195134} (2019)

















\bibitem{mermin_dft} N.D.~Mermin, Thermal Properties of the Inhomogeneous Electron Gas, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.137.A1441}{\textit{Phys.~Rev.}~\textbf{137}, A1441} (1965)

\bibitem{rajagopal_dft} U.~Gupta and A.K.~Rajagopal, Density functional formalism at finite temperatures with some applications, \href{https://www.sciencedirect.com/science/article/pii/0370157382900771}{\textit{Phys.~Reports} \textbf{87}, 259-311} (1982)





\bibitem{kushal} K.~Ramakrishna, T.~Dornheim, and J.~Vorberger, Influence of finite temperature Exchange-Correlation effects in Hydrogen, \href{https://arxiv.org/abs/2002.11574}{arxiv:2002.11574} (submitted for publication)





\bibitem{kugler1} A.A.~Kugler, Theory of the Local Field Correction in an Electron Gas, \href{ http://link.springer.com/article/10.1007/BF01024183}{ \textit{J.~Stat.~Phys.}~\textbf{12}, 35} (1975)















% advanced functionals for DFT

\bibitem{burke_ac} A.~Pribram-Jones, P.E.~Grabowski, and K.~Burke, Thermal Density Functional Theory: Time-Dependent Linear Response and Approximate Functionals from the Fluctuation-Dissipation Theorem, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.116.233001}{\textit{Phys.~Rev.~Lett.}~\textbf{116}, 233001} (2016)

\bibitem{lu_ac} D.~Lu, Evaluation of model exchange-correlation kernels in the adiabatic connection fluctuation-dissipation theorem for inhomogeneous systems, \href{https://aip.scitation.org/doi/10.1063/1.4867538}{\textit{J.~Chem.~Phys.}~\textbf{140}, 18A520} (2014)

\bibitem{patrick_ac} C.E.~Patrick and K.S.~Thygesen, Adiabatic-connection fluctuation-dissipation DFT for the structural properties of solids—The renormalized ALDA and electron gas kernels, \href{https://aip.scitation.org/doi/10.1063/1.4919236}{\textit{J.~Chem.~Phys.}~\textbf{143}, 102802} (2015)

\bibitem{goerling_ac} A.~G\"orling, Hierarchies of methods towards the exact Kohn-Sham correlation energy based on the adiabatic-connection fluctuation-dissipation theorem, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.235120}{\textit{Phys.~Rev.~B} \textbf{99}, 235120} (2019)






\bibitem{without_chihara} A.D.~Baczewski, L.~Shulenburger, M.P.~Desjarlais, S.B.~Hansen, and R.J.~Magyar, X-ray Thomson Scattering in Warm Dense Matter without the Chihara Decomposition, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.116.115004}{\textit{Phys.~Rev.~Lett.}~\textbf{116}, 115004} (2016)











\bibitem{diaw1} A.~Diaw and M.S.~Murillo, Generalized hydrodynamics model for strongly coupled plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.92.013107}{\textit{Phys.~Rev.~E} \textbf{92}, 013107} (2015)

\bibitem{diaw2} A.~Diaw and M.S.~Murillo, A viscous quantum hydrodynamics model based on dynamic density functional theory, \href{https://www.nature.com/articles/s41598-017-14414-9}{\textit{Sci.~Reports}~\textbf{7}, 15352} (2017)

\bibitem{zhanods_hydro} Zh.A.~Moldabekov, M.~Bonitz, and T.S.~Ramazanov, Theoretical foundations of quantum hydrodynamics for plasmas, \href{https://aip.scitation.org/doi/abs/10.1063/1.5003910}{\textit{Phys.~Plasmas} \textbf{25}, 031903} (2018)












\bibitem{ceperley_potential} G.~Senatore, S.~Moroni, and D.M.~Ceperley, Local field factor and effective potentials in liquid metals, \href{https://www.sciencedirect.com/science/article/pii/S002230939600316X}{\textit{J.~Non-Cryst.~Sol.}~\textbf{205-207}, 851-854} (1996)


\bibitem{zhandos1} Zh.A.~Moldabekov, S.~Groth, T.~Dornheim, H.~K\"ahlert, M.~Bonitz, and T.S.~Ramazanov, Structural characteristics of strongly coupled ions in a dense quantum plasma, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.98.023207}{\textit{Phys.~Rev.~E} \textbf{98}, 023207} (2018)

\bibitem{zhandos2} Zh.A.~Moldabekov, H.~K\"ahlert, T.~Dornheim, S.~Groth, M.~Bonitz, and T.S.~Ramazanov, Dynamical structure factor of strongly coupled ions in a dense quantum plasma, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.99.053203}{\textit{Phys.~Rev.~E} \textbf{99}, 053203} (2019)









\bibitem{siegfried_review} S.H.~Glenzer and R.~Redmer, X-ray Thomson scattering in high energy density plasmas, \href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.81.1625}{\textit{Rev.~Mod.~Phys.}~\textbf{81}, 1625} (2009)




\bibitem{kraus_xrts} D.~Kraus, B.~Bachmann, B.~Barbrel, R.W.~Falcone, L.B.~Fletcher, S.~Frydrych, E.J.~Gamboa, M.~Gauthier, D.O.~Gericke, S.H.~Glenzer, S.~G\"ode, E.~Granados, N.J.~Hartley, J.~Helfrich, H.J.~Lee, B.~Nagler, A.~Ravasio, W.~Schumaker, J.~Vorberger, and T.~D\"oppner, Characterizing the ionization potential depression in dense carbon plasmas with high-precision spectrally resolved x-ray scattering, \href{https://iopscience.iop.org/article/10.1088/1361-6587/aadd6c/meta}{\textit{Plasma Phys.~Control Fusion} \textbf{61}, 014015} (2019)






\bibitem{stopping2} D.O.~Gericke, M.~Schlanges, and W.D.~Kraeft, Stopping power of a quantum plasma---T-matrix approximation and dynamical screening, \href{https://www.sciencedirect.com/science/article/pii/0375960196006548}{\textit{Phys.~Lett.~A} \textbf{222}, 241-245} (1996)

\bibitem{stopping} Zh.A.~Moldabekov, T.~Dornheim, M.~Bonitz, and T.S.~Ramazanov, Ion energy loss characteristics and friction in a free electron gas at warm dense matter and non-ideal dense plasma conditions, 
\href{https://link.aps.org/doi/10.1103/PhysRevE.101.053203}{\textit{Phys. Rev. E} \textbf{101}, 053203} (2020)



\bibitem{Desjarlais:2017}
M.P.~Desjarlais, P.~Michael C.R.~Scullard, L.X.~Benedict, H.D.~Whitley, and R.~Redmer,
Density-functional calculations of transport properties in
the nondegenerate limit and the role of electron-electron scattering
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.95.033203}{\textit{Phys. Rev. E} \textbf{95}, 033203} (2017)


\bibitem{Veysman:2016} M.~Veysman, G.~R\"opke, M.~Winkel, and H.~Reinholz, Optical conductivity of warm dense matter within a wide
frequency range using quantum statistical and kinetic approaches
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.94.013203}{\textit{Phys. Rev. E},
  \textbf{94}, 013203} (2016)








\bibitem{jan_relax} J.~Vorberger, D.O.~Gericke, Th.~Bornath, and M.~Schlanges, Energy relaxation in dense, strongly coupled two-temperature plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.81.046404}{\textit{Phys.~Rev.~E} \textbf{81}, 046404} (2010)





\bibitem{moroni} S.~Moroni, D.M.~Ceperley, and G.~Senatore, 
Static response from quantum Monte Carlo calculations, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.69.1837}{\textit{Phys.~Rev.~Lett.}~\textbf{69}, 1837} (1992)









\bibitem{dynamic_folgepaper} S.~Groth, T.~Dornheim, and J.~Vorberger, \textit{Ab Initio} Path Integral Monte Carlo Approach to the Static and Dynamic Density Response of the Uniform Electron Gas, \href{https://link.aps.org/doi/10.1103/PhysRevB.99.235122}{\textit{Phys.~Rev.~B} \textbf{99}, 235122} (2019)



\bibitem{dornheim_ML} T.~Dornheim, J.~Vorberger, S.~Groth, N.~Hoffmann, Zh.A.~Moldabekov, and M.~Bonitz, The Static Local Field Correction of the Warm Dense Electron Gas: An ab Initio Path Integral Monte Carlo Study and Machine Learning Representation, \textit{J.~Chem.~Phys.}~(in press), \href{https://arxiv.org/abs/1907.08473}{arxiv:1907.08473}
























\bibitem{cdop} M.~Corradini, R.~Del Sole, G.~Onida, and M.~Palummo, Analytical Expressions for the Local-Field Factor $G(q)$ and the Exchange-Correlation Kernel ${K}_{\mathrm{xc}}(r)$ of the Homogeneous Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevB.57.14569}{ \textit{Phys.~Rev.~B} \textbf{57}, 14569} (1998)



% Parametrization of ground state properties





\bibitem{dornheim_EL} T.~Dornheim, T.~Sjostrom, S.~Tanaka, and J.~Vorberger, Strongly coupled electron liquid: Ab initio path integral Monte Carlo simulations and dielectric theories, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.101.045129}{\textit{Phys.~Rev.~B} \textbf{101}, 045129} (2020)

\bibitem{dornheim_HED} T.~Dornheim, Zh.A.~Moldabekov, J.~Vorberger, and S.~Groth, Ab initio path integral Monte Carlo simulation of the Uniform Electron Gas in the High Energy Density Regime, (Plasma Phys.~Control.~Fusion, in press)




\bibitem{dornheim_nonlinear} T.~Dornheim, J.~Vorberger, and M.~Bonitz, Nonlinear Electronic Density Response in Warm Dense Matter, \href{https://arxiv.org/abs/2004.03229}{arXiv:2004.03229} (submitted for publication)









\bibitem{dynamic_sign_problem} M.~Schiro, Real-time dynamics in quantum impurity models with diagrammatic Monte Carlo, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.81.085126}{\textit{Phys.~Rev.~B} \textbf{81}, 085126} (2010)

\bibitem{dynamic_sign_problem2} C.H.~Mak and R.~Egger, A multilevel blocking approach to the sign problem in real-time quantum Monte Carlo simulations, \href{https://aip.scitation.org/doi/abs/10.1063/1.478077}{\textit{J.~Chem.~Phys.}~\textbf{110}, 12} (1999)






\bibitem{kwong} N.-H.~Kwong and M.~Bonitz, Real-Time Kadanoff-Baym Approach to Plasma Oscillations in a Correlated Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.84.1768}{\textit{Phys.~Rev.~Lett.}~\textbf{84}, 1768} (2000)








\bibitem{takada1} Y.~Takada and H.~Yasuhara, Dynamical Structure Factor of the Homogeneous Electron Liquid: Its Accurate Shape and the Interpretation of Experiments on Aluminum, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.89.216402}{\textit{Phys.~Rev.~Lett.}~\textbf{89}, 216402} (2002)


\bibitem{takada2} Y.~Takada, Emergence of an excitonic collective mode in the dilute electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.94.245106}{\textit{Phys.~Rev.~B}~\textbf{94}, 245106} (2016)
































\bibitem{jarrell} M.~Jarrell and J.E.~Gubernatis, Bayesian inference and the analytic continuation of imaginary-time quantum Monte Carlo data, \href{https://www.sciencedirect.com/science/article/abs/pii/0370157395000747}{\textit{Phys.~Reports}~\textbf{269}, 133-195} (1996)


\bibitem{mem_revisited} Y.~Kora and M.~Boninsegni, Dynamic structure factor of superfluid $^4$He from quantum Monte Carlo: Maximum entropy revisited, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.98.134509}{\textit{Phys.~Rev.~B} \textbf{98}, 134509} (2018)

\bibitem{gift} E.~Vitali, M.~Rossi, and D.E.~Galli, \textit{Ab initio} low-energy dynamics of superfluid and solid $^4$He, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.82.174510}{\textit{Phys.~Rev.~B} \textbf{82}, 174510} (2010)

\bibitem{gift2} G.~Bertaina, D.E.~Galli, and E.~Vitali, Statistical and computational intelligence approach to analytic continuation in Quantum Monte Carlo, \href{https://www.tandfonline.com/doi/full/10.1080/23746149.2017.1288585}{\textit{Adv.~in Phys.: X} \textbf{2}, 302-329} (2017)

















\bibitem{dornheim_dynamic} T.~Dornheim, S.~Groth, J.~Vorberger, and M.~Bonitz, \textit{Ab initio} Path Integral Monte Carlo Results for the Dynamic Structure Factor of Correlated Electrons: From the Electron Liquid to Warm Dense Matter, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.121.255001}{\textit{Phys.~Rev.~Lett.}~\textbf{121}, 255001} (2018)














\bibitem{imada} M.~Takahashi and M.~Imada, Monte Carlo Calculation of Quantum Systems, \href{https://www.jstage.jst.go.jp/article/jpsj1946/53/3/53_3_963/_article/-char/ja/}{\textit{J.~Phys.~Soc.~Jpn.}~\textbf{53}, 963} (1984)

\bibitem{cep} D.M.~Ceperley, Path integrals in the theory of condensed helium, \href{http://link.aps.org/doi/10.1103/RevModPhys.67.279}{\textit{Rev. Mod. Phys.} \textbf{67}, 279-355} (1995)







\bibitem{trotter} H.~de Raedt and B.~de Raedt, Applications of the generalized Trotter formula, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.28.3575}{\textit{Phys.~Rev.~A} \textbf{28}, 3575} (1983)



\bibitem{HO1} L.~Brualla, K.~Sakkos, J.~Boronat, and J.~Casulleras, Higher order and infinite Trotter-number extrapolations in path integral Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.1760512}{\textit{J.~Chem.~Phys.}~\textbf{121}, 636} (2004)

\bibitem{HO2} K.~Sakkos, J.~Casulleras, and J.~Boronat, High order Chin actions in path integral Monte Carlo, \href{https://aip.scitation.org/doi/full/10.1063/1.3143522}{\textit{J.~Chem.~Phys.}~\textbf{130}, 204109} (2009)










% Vanilla ground-state DFT review





\bibitem{groth_cpp} S.~Groth, T.~Dornheim, and M.~Bonitz, Free energy of the uniform electron gas: Testing analytical models against first‐principles results, \href{https://onlinelibrary.wiley.com/doi/abs/10.1002/ctpp.201600082}{\textit{Contrib.~Plasma Phys.}~\textbf{57}, 137-146} (2017)



















































































\bibitem{stls} S.~Tanaka and S.~Ichimaru, Thermodynamics and Correlational Properties of Finite-Temperature Electron Liquids in the Singwi-Tosi-Land-Sj\"olander Approximation, \href{ http://journals.jps.jp/doi/abs/10.1143/JPSJ.55.2278 }{ \textit{J.~Phys.~Soc.~Jpn.}~\textbf{55}, 2278-2289} (1986)


\bibitem{stls2} T.~Sjostrom, and J.~Dufty, Uniform Electron Gas at Finite Temperatures, \href{ http://link.aps.org/doi/10.1103/PhysRevB.88.115123 }{ \textit{Phys.~Rev.~B} \textbf{88}, 115123} (2013)



\bibitem{stls_original} K.S.~Singwi, M.P.~Tosi, R.H.~Land, and A.~Sj\"olander, Electron Correlations at Metallic Densities, \href{ http://link.aps.org/doi/10.1103/PhysRev.176.589}{ \textit{Phys.~Rev.}~\textbf{176}, 589} (1968)



\bibitem{vs_original} P.~Vashishta, and K.S.~Singwi, Electron Correlations at Metallic Densities. V, \href{ http://link.aps.org/doi/10.1103/PhysRevB.6.875}{ \textit{Phys.~Rev.~B} \textbf{6}, 875 } (1972)








\bibitem{tanaka_hnc} S.~Tanaka, Correlational and thermodynamic properties of finite-temperature electron liquids in the hypernetted-chain approximation, \href{https://aip.scitation.org/doi/abs/10.1063/1.4969071}{\textit{J.~Chem.~Phys.}~\textbf{145}, 214104} (2016)














\bibitem{dornheim_permutation_cycles} T.~Dornheim, S.~Groth, A.~Filinov, and M.~Bonitz, Path Integral Monte Carlo Simulation of Degenerate Electrons: Permutation-Cycle Properties, \href{https://aip.scitation.org/doi/10.1063/1.5093171}{\textit{J.~Chem.~Phys.}~\textbf{151}, 014108} (2019)













\bibitem{metropolis} N.~Metropolis, A.W.~Rosenbluth, M.N.~Rosenbluth, A.H.~Teller, and E.~Teller, Equation of State Calculations by Fast Computing Machines, \href{https://aip.scitation.org/doi/abs/10.1063/1.1699114}{\textit{J.~Chem.~Phys.}~\textbf{21}, 1087} (1953)
















\bibitem{velocity} E.~Rabani, D.R.~Reichman, G.~Krilov, and B.J.~Berne, The calculation of transport properties in quantum liquids using the maximum entropy numerical analytic continuation method: Application to liquid para-hydrogen, \href{https://www.pnas.org/content/99/3/1129}{\textit{PNAS} \textbf{99}, 1129-1133} (2002)



\bibitem{mezza} F.~Mezzacapo and M.~Boninsegni, Structure, superfluidity, and quantum melting of hydrogen clusters, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.75.033201}{\textit{Phys.~Rev.~A} \textbf{75}, 033201} (2007)





\bibitem{boninsegni1} M.~Boninsegni, N.V.~Prokofev, and B.V.~Svistunov, Worm algorithm and diagrammatic Monte Carlo: A new approach to continuous-space path integral Monte Carlo simulations, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.74.036701}{\textit{Phys.~Rev.~E}~\textbf{74}, 036701} (2006)

\bibitem{boninsegni2} M.~Boninsegni, N.V.~Prokofev, and B.V.~Svistunov, Worm Algorithm for Continuous-Space Path Integral Monte Carlo Simulations, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.96.070601}{\textit{Phys.~Rev.~Lett.}~\textbf{96}, 070601} (2006)












\bibitem{vanLeeuwen} G.~Stefanucci and R.~van Leeuwen, Nonequilibrium Many-Body Theory of Quantum Systems: A Modern Introduction, Cambridge University Press, Cambridge, United Kingdom, 2013







\bibitem{stls_1985} S.~Tanaka, S.~Mitake, and S.~Ichimaru, Parametrized equation of state for electron liquids in the Singwi-Tosi-Land-Sj\"olander approximation, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.32.1896}{\textit{Phys.~Rev.~A} \textbf{32}, 1896} (1985)









\bibitem{dynamic_i} T.~Hasegawa and M.~Shimizu, Electron correlations at metallic densities, II. Quantum mechanical expression of dielectric function with Wigner distribution function, \href{https://www.jstage.jst.go.jp/article/jpsj1946/38/4/38_4_965/_article/-char/ja/}{\textit{J.~Phys.~Soc.~Jpn.}~\textbf{38}, 965} (1975)




\bibitem{dynamic_iii} R.K.~Moudgil, P.K.~Ahluwalia, and K.N.~Pathak, Static and dynamic correlation functions of a two-dimensional quantum electron fluid, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.52.11945}{\textit{Phys.~Rev.~B} \textbf{52}, 11945} (1995)









\bibitem{arora} P.~Arora, K.~Kumar, and R.K.~Moudgil, Spin-resolved correlations in the warm-dense homogeneous electron gas, \href{https://link.springer.com/article/10.1140/epjb/e2017-70532-y}{\textit{Eur.~Phys.~J.~B}~\textbf{90}, 76} (2017)





\bibitem{stolzmann} W.~Stolzmann and M.~R\"osler, Static Local-Field Corrected Dielectric and Thermodynamic Functions, \href{ http://onlinelibrary.wiley.com/doi/10.1002/1521-3986(200103)41:2/3<203::AID-CTPP203>3.0.CO;2-S/abstract }{ \textit{Contrib.~Plasma Phys.}~\textbf{41}, 203} (2001)







\bibitem{lkw_fahrer} Zh.A.~Moldabekov, S.~Groth, T.~Dornheim, H.~K\"ahlert, M.~Bonitz, and T.S.~Ramazanov, Structural characteristics of strongly coupled ions in a dense quantum plasma, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.98.023207}{\textit{Phys.~Rev.~E} \textbf{98}, 023207} (2018)






\bibitem{bowen} G.~Sugiyama, C.~Bowen, and B.J.~Alder, Static dielectric response of charged bosons, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.46.13042}{\textit{Phys.~Rev.~B}~\textbf{46}, 13042} (1992)







\bibitem{bowen2} C.~Bowen, G.~Sugiyama, and B.J.~Alder, Static Dielectric Response of the Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevB.50.14838}{\textit{Phys.~Rev.~B} \textbf{50}, 14838} (1994)










% Our primitive static response approach!


\bibitem{dornheim_pre} T.~Dornheim, S.~Groth, J.~Vorberger, and M.~Bonitz, Permutation Blocking Path Integral Monte Carlo approach to the Static Density Response of the Warm Dense Electron Gas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.96.023203}{\textit{Phys.~Rev.~E}~\textbf{96}, 023203} (2017)

\bibitem{groth_jcp} S.~Groth, T.~Dornheim, and M.~Bonitz, Configuration Path Integral Monte Carlo approach to the Static Density Response of the Warm Dense Electron Gas, \href{https://aip.scitation.org/doi/abs/10.1063/1.4999907}{\textit{J.~Chem.~Phys.}~\textbf{147}, 164108} (2017)











\bibitem{berne1} D.~Thirumalai and B.J.~Berne, On the calculation of time correlation functions in quantum systems: Path integral techniques, \href{https://aip.scitation.org/doi/abs/10.1063/1.445597}{\textit{J.~Chem.~Phys.}~\textbf{79}, 5029} (1983)


\bibitem{berne2} E.~Gallicchio and B.J.~Berne, The absorption spectrum of the solvated electron in fluid helium by maximum entropy inversion of imaginary time correlation functions from path integral Monte Carlo simulations, \href{https://aip.scitation.org/doi/abs/10.1063/1.467892}{\textit{J.~Chem.~Phys.}~\textbf{101}, 9909} (1994)














\bibitem{fraser} L.M.~Fraser, W.M.C.~Foulkes, G.~Rajagopal, R.J.~Needs, S.D.~Kenny, and A.J.~Williamson, Finite-size effects and Coulomb interactions in quantum Monte Carlo calculations for homogeneous systems with periodic boundary conditions, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.53.1814}{\textit{Phys.~Rev.~B} \textbf{53}, 1814} (1996)


\bibitem{chiesa} S.~Chiesa, D.M.~Ceperley, R.M.~Martin, and M.~Holzmann, Finite-Size Error in Many-Body Simulations with Long-Range Interactions, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.97.076404}{\textit{Phys.~Rev.~Lett.}~\textbf{97}, 076404} (2006)

\bibitem{drummond} N.D.~Drummond, R.J.~Needs, A.~Sorouri, and W.M.C.~Foulkes, Finite-size errors in continuum quantum Monte Carlo calculations, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.78.125106}{\textit{Phys.~Rev.~B} \textbf{78}, 125106} (2008)


\bibitem{holzmann} M.~Holzmann, R.C.~Clay III, M.A.~Morales, N.M.~Tubman, D.M.~Ceperley, and C.~Pierleoni, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.94.035126}{\textit{Phys.~Rev.~B} \textbf{94}, 035126} (2016)













% ### Exciting new developments in the field of fermionic QMC simulations:




\bibitem{kugler_bounds} A.A.~Kugler, Bounds for Some Equilibrium Properties of an Electron Gas, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.1.1688}{\textit{Phys.~Rev.~A} \textbf{1}, 1688} (1970)






\bibitem{github_link} A link to a GitHub repository containing the PIMC data will be made available upon publication.









\bibitem{holas_limit} A.~Holas, Exact asymptotic expression for the static dielectric function of a uniform electron liquid at large wave vector,  in Strongly Coupled Plasma Physics, edited by F.J.~Rogers and H.E.~DeWitt (Plenum,NewYork,1987), p.46



\bibitem{negative_kxc_note} It is well known~\cite{neg1,neg2,stls} that $K_\text{xc}$ becomes negative for weak coupling above a certain temperature. Indeed, the negative large-$q$ asymptote of $G(q)$ predicted by Eq.~(\ref{eq:TAIL}) has recently been reported in this regime, see Ref.~\cite{dornheim_ML}.


\bibitem{neg1} B.~Militzer and E.L.~Pollock, Lowering of the Kinetic Energy in Interacting Quantum Systems, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.89.280401}{\textit{Phys.~Rev.~Lett.}~\textbf{89}, 280401} (2002)

\bibitem{neg2} W.D.~Kraeft, M.~Schlanges, J.~Vorberger, and H.E.~DeWitt, Kinetic and correlation energies and distribution functions of dense plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.66.046405}{\textit{Phys.~Rev.~E} \textbf{66}, 046405} (2002)




\bibitem{iyetomi_review} S.~Ichimaru, H.~Iyetomi, and S.~Tanaka, Statistical physics of dense plasmas: thermodynamics, transport coefficients and dynamic correlations, \href{https://www.sciencedirect.com/science/article/pii/0370157387901256}{\textit{Phys.~Reports} \textbf{149}, 91-205} (1987)







\bibitem{farid} B.~Farid, V.~Heine, G.E.~Engel, and I.J.~Robertson, Extremal Properties of the Harris-Foulkes Functional and an Improved Screening Calculation for the Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevB.48.11602}{\textit{Phys.~Rev.~B} \textbf{48}, 11602} (1993) 

\bibitem{kimball} J.C.~Kimball, Short-Range Correlations and Electron-Gas Response Functions, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.7.1648}{\textit{Phys.~Rev.~A} \textbf{7}, 1648} (1973)

\bibitem{bonitz_book} M. Bonitz, Quantum Kinetic Theory, 2nd ed. Springer 2016.

\bibitem{alexandrov_book} Alexandrov, Bogdankievich, Rukhadse, Plasma Electrodynamics











%\bibitem{feynman} R.P.~Feynman and A.R.~Hibbs, Quantum Mechanics and Path Integrals, Dover Publications, New York (2010)


%\bibitem{chandler} D.~Chandler and P.G.~Wolynes, Exploiting the isomorphism between quantum theory and classical statistical mechanics of polyatomic fluids, \href{https://aip.scitation.org/doi/abs/10.1063/1.441588}{\textit{J.~Chem.~Phys.}~\textbf{74}, 4078} (1981)


%\bibitem{kleinert} H.~Kleinert, Path Integrals in Quantum Mechanics, Statistics, Polymer Physics, and Financial Markets, World Scientific, Singapore, 2009









%\bibitem{curse} A.~Hinrichs, E.~Novak, M.~Ullrich and H.~Wozniakowski, The curse of dimensionality for numerical integration of smooth functions, \href{http://www.ams.org/journals/mcom/2014-83-290/S0025-5718-2014-02855-X/home.html}{\textit{Math.~Comp.}~\textbf{83}, 2853-2863} (2014)


%\bibitem{filinov_chapter} A.~Filinov and M.~Bonitz, Classical and Quantum Monte Carlo, \textit{Introduction to Computational Methods in Many Body Physic}, M.~Bonitz and D.~Semkat (Eds.), Rinton Press, Paramus (New Jersey) (2006)

%\bibitem{liu_monte_carlo} J.~Liu, Monte Carlo Strategies in Scientific Computing, Springer, New York (2013)


%\bibitem{pimc_original} L.D.~Fosdick and H.F.~Jordan, Path-Integral Calculation of the Two-Particle Slater Sum for He$^4$, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.143.58}{\textit{Phys.~Rev.}~\textbf{143}, 58} (1966)

%\bibitem{pimc_original2} H.F.~Jordan and L.D.~Fosdick, Three-Particle Effects in the Pair Distribution Function for He$^4$ Gas, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.171.128}{\textit{Phys.~Rev.}~\textbf{171}, 128} (1968)













% ### Crystal

%\bibitem{jones_crystal} M.D.~Jones and D.M.~Ceperley, Crystallization of the one-component plasma at finite temperature, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.76.4572}{\textit{Phys.~Rev.~Lett.}~\textbf{76}, 4572} (1996)


%\bibitem{filinov_PRL} A.V.~Filinov, M.~Bonitz, and Yu.E.~Lozovik, Wigner Crystallization in Mesoscopic 2D Electron Systems, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.86.3851}{\textit{Phys.~Rev.~Lett.}~\textbf{86}, 3851} (2001)













% ### Path Integral Monte Carlo (worm algorithm)


















%\bibitem{ceperley_fermions} D.M.~Ceperley, Path Integral Monte Carlo Methods for Fermions, \textit{Monte Carlo and Molecular Dynamics of Condensed Matter Systems}, K.~Binder and G.~Ciccotti (Eds.), Bologna (Italy) (1996)

























%\bibitem{wigner_molecule1} S.M.~Reimann, M.~Koskinen, and M.~Manninen, Formation of Wigner molecules in small quantum dots, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.62.8108}{\textit{Phys.~Rev.~B}~\textbf{62}, 8108} (2000)

%\bibitem{wigner_molecule2} B.~Reusch, W.~H\"ausler, and H.~Grabert, Wigner molecules in quantum dots, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.63.113313}{\textit{Phys.~Rev.~B}~\textbf{63}, 113313} (2001)

%\bibitem{wigner_molecule3} E.~R\"as\"anen, H.~Saarikoski, M.J.~Puska, and R.M.~Nieminen, Wigner molecules in polygonal quantum dots: A density-functional study, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.67.035326}{\textit{Phys.~Rev.~B}~\textbf{87}, 035326} (2003)




%\bibitem{ross} M.~Ross, Matter under extreme conditions of temperature and pressure, \href{https://doi.org/10.1088\%2F0034-4885\%2F48\%2F1\%2F001}{\textit{Rep.~Prog.~Phys.}~\textbf{48}, 1--52} (1985)

%\bibitem{koenig} M.~Koenig \textit{et al.}, Progress in the study of warm dense matter, \href{https://doi.org/10.1088\%2F0741-3335\%2F47\%2F12b\%2Fs31}{\textit{Plasma Phys.~Control.~Fusion} \textbf{47}, B441--B449} (2005)



%\bibitem{fortov_review} V.E.~Fortov, Extreme states of matter on Earth and in space, \href{https://www.turpion.org/php/paper.phtml?journal_id=pu&paper_id=6821}{\textit{Phys.-Usp.}~\textbf{52}, 615--647} (2009)















%\bibitem{brown_chapter} E.~Brown, M.A.~Morales, C.~Pierleoni, and D.~Ceperley, Quantum Monte Carlo Techniques and Applications for Warm Dense
%Matter, in F. Graziani, M. P. Desjarlais, R. Redmer, and S. B.
%Trickey (Eds.), \textit{Frontiers and Challenges in Warm Dense Matter},
%Springer International Publishing (2014)



































%\bibitem{brenda} Y.~Liu, M.~Cho, and B.~Rubenstein, \textit{Ab Initio} Finite Temperature Auxiliary Field Quantum Monte Carlo, \href{https://pubs.acs.org/doi/abs/10.1021/acs.jctc.8b00569}{\textit{J.~Chem.~Theory~Comput.}~\textbf{14}, 4722-4732} (2018)


%\bibitem{universe} V.~Filinov and A.~Larkin, Quantum Dynamics of Charged Fermions in the Wigner Formulation of Quantum Mechanics, \href{https://www.mdpi.com/2218-1997/4/12/133/htm}{\textit{Universe} \textbf{4}, 133} (2018)












%\bibitem{trotter} H.~De Raedt and B.~De Raedt, Applications of the generalized Trotter formula, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.28.3575}{\textit{Phys.~Rev.~A} \textbf{28}, 3575} (1983)






%\bibitem{fermion_nodes} D.M.~Ceperley, Fermion nodes, \href{https://link.springer.com/article/10.1007/BF01030009}{\textit{J.~Stat.~Phys.}~\textbf{63}, 1237-1267} (1991)









%\bibitem{dornheim_analyzing} T.~Dornheim, H.~Thomsen, P.~Ludwig, A.~Filinov, and M.~Bonitz, Analyzing Quantum Correlations Made Simple, \href{https://onlinelibrary.wiley.com/doi/abs/10.1002/ctpp.201500120}{\textit{Contrib.~Plasma Phys.}~\textbf{56}, 371-379} (2016)






%\bibitem{reimann} S.M.~Reimann and M.~Manninen, Electronic structure of quantum dots, \href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.74.1283}{\textit{Rev.~Mod.~Phys.}~\textbf{74}, 1283} (2002)





















%\bibitem{stuhler} J. Stuhler, A. Griesmaier, T. Koch, M. Fattori, T. Pfau, S. Giovanazzi, P. Pedri, and L. Santos, Observation of Dipole-Dipole Interaction in a Degenerate Quantum Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.95.150406}{\textit{Phys.~Rev.~Lett.}~\textbf{95}, 150406} (2005)

\bibitem{dynamic_alex1} A.~Filinov and M.~Bonitz, Collective and single-particle excitations in two-dimensional dipolar Bose gases, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.86.043628}{\textit{Phys.~Rev.~A} \textbf{86}, 043628} (2012)





%\bibitem{jan_willem} J.W.~Abraham and M.~Bonitz, Quantum Breathing Mode of Trapped Particles: From Nanoplasmas to Ultracold Gases, \href{https://onlinelibrary.wiley.com/doi/abs/10.1002/ctpp.201300066}{\textit{Contrib.~Plasma Phys.}~\textbf{54}, 27-99} (2014)






















% ### The UEG in general















%\bibitem{brualla} L.~Brualla, K.~Sakkos, J.~Boronat, and J.~Casulleras, Higher order and infinite Trotter-number extrapolationsin path integral Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.1760512}{\textit{J.~Chem.~Phys.}~\textbf{121}, 636} (2004)

%\bibitem{sakkos} K.~Sakkos, J.~Casulleras, and J.~Boronat, High order Chin actions in path integral Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.3143522}{\textit{J.~Chem.~Phys.}~\textbf{130}, 204109} (2009)










%\bibitem{monte_carlo_book} G.~Fishman, Monte Carlo, \textit{Springer Series in Operations Research and Financial Engineering}, Springer, New York (1996)


























% benchmarking and guiding the development of new methods

\bibitem{panholzer1} M.~Panholzer, R.~Hobbiger, and H.~B\"ohm, Optimized correlations inspired by perturbation theory, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.195156}{\textit{Phys.~Rev.~B} \textbf{99}, 195156} (2019)




\bibitem{clark_casula} B.K.~Clark, M.~Casula, and D.M.~Ceperley, Hexatic and Mesoscopic Phases in a 2D Quantum Coulomb System, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.103.055701}{\textit{Phys.~Rev.~Lett.}~\textbf{103}, 055701} (2009)



%\bibitem{krauth_book} W.~Krauth,
%Statistical  Mechanics: Algorithms  and  Computations, \textit{Oxford Master Series in Physics}, Oxford University Press, 2006










\bibitem{dynamic_alex2} A.~Filinov, Correlation effects and collective excitations in bosonic bilayers: Role of quantum statistics, superfluidity, and the dimerization transition, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.94.013603}{\textit{Phys.~Rev.~A} \textbf{94}, 013603} (2016)











%\bibitem{greiner_book} W.~Greiner, D.~Rischke, L.~Neise, and H.~St\"ocker, Thermodynamics and Statistical Mechanics, Springer, New York (2012)


%\bibitem{janke} W.~Janke and T.~Sauer, Optimal energy estimation in path-integral Monte Carlo simulations, \href{https://aip.scitation.org/doi/abs/10.1063/1.474309}{\textit{J.~Chem.~Phys.}~\textbf{107}, 5821} (1997)






























% ### Here we introduce the frequency moments and stuff:

\bibitem{iwamoto2} N~Iwamoto, Inequalities for frequency-moment sum rules of electron liquids, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.33.1940}{\textit{Phys.~Rev.}~A \textbf{33}, 1940} (1985)


\bibitem{pines_woo} D.~Pines and C.-W. Woo, Sum Rules, Structure Factors, and Phonon Dispersion in Liquid $^4$He at Long Wavelengths and Low Temperatures, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.24.1044}{\textit{Phys.~Rev.~Lett.}~\textbf{24}, 1044} (1970)



\bibitem{kugler2} A.A.~Kugler, Bounds for Some Equilibrium Properties of an Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevA.1.1688}{ \textit{Phys.~Rev.~A} \textbf{1}, 1688} (1970)




\bibitem{puff1} R.D.~Puff, Application of Sum Rules to the Low-Temperature Interacting Boson System, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.137.A406}{\textit{Phys.~Rev.}~\textbf{137}, A406} (1965)

\bibitem{puff2} N.~Mihara and R.D.~Puff, Liquid Structure Factor of Ground-State He$^4$, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.174.221}{\textit{Phys.~Rev.}~\textbf{174}, 221} (1968)




\bibitem{iwamoto} N.~Iwamoto, E.~Krotscheck, and D.~Pines, Theory of electron liquids. II. Static and dynamic form factors, correlation energy, and plasmon dispersion, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.29.3936}{\textit{Phys.~Rev.~B}~\textbf{29}, 3936} (1984)








\bibitem{dabrowski} B.~Dabrowski, Dynamical local-field factor in the response function of an electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.34.4989}{\textit{Phys.~Rev.~B}~\textbf{34}, 4989} (1986)








% Inserted by TD, to be sorted.


\bibitem{dornheim_FSC} T.~Dornheim and J.~Vorberger, Finite-size effects in the reconstruction of dynamic properties from ab initio path integral Monte-Carlo simulations, \href{https://arxiv.org/abs/2004.13429}{arxiv:2004.13429}


\bibitem{higuchi} M.~Highuchi and H.~Yasuhara, 
Kleinman's Dielectric Function and Interband Optical Absorption Strength of Simple Metals, \href{https://journals.jps.jp/doi/abs/10.1143/JPSJ.69.2099}{\textit{J.~Phys.~Soc.~Jpn.}~\textbf{69} 2099-2106} (2000)
 



\bibitem{Zastrau}
U. Zastrau, P. Sperling, M. Harmand, A. Becker, T. Bornath, R. Bredow, S. Dziarzhytski, T. Fennel,
L. B. Fletcher, E. Förster, S. Göde, G. Gregori, V. Hilbert, D. Hochhaus, B. Holst, T. Laarmann,
H. J. Lee, T. Ma, J. P. Mithen, R. Mitzner, C.D. Murphy, M. Nakatsutsumi, P. Neumayer, A. Przystawik,
S. Roling, M. Schulz, B. Siemer, S. Skruszewicz, J. Tiggesbäumker, S. Toleikis, T. Tschentscher,
T. White, M. Wöstmann, H. Zacharias, T. Döppner, S. H. Glenzer, and R. Redmer,
Resolving ultrafast heating of dense cryogenic hydrogen
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.112.105002}{\textit{Phys. Rev. Lett.}~\textbf{112}, 105002}  (2014)




\bibitem{benage} J.F.~Benage, W.R.~Shanahan, and M.S.~Murillo, Electrical Resistivity Measurements of Hot Dense Aluminum, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.83.2953}{\textit{Phys.~Rev.~Lett.}~\textbf{83}, 2953} (1999)


\bibitem{karasiev_importance} V.V.~Karasiev, L.~Calderin, and S.B.~Trickey, Importance of finite-temperature exchange correlation for warm dense matter calculations, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.93.063207}{\textit{Phys.~Rev.~E} \textbf{93}, 063207} (2016)



\bibitem{low_density1} S. Mazevet, M. P. Desjarlais, L. A. Collins, J. D. Kress, and N. H. Magee, Simulations of the optical properties of warm dense aluminum, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.71.016409}{\textit{Phys.~Rev.~E} \textbf{71}, 016409} (2005)

\bibitem{low_density2} M. P. Desjarlais, J. D. Kress, and L. A. Collins, Electrical conductivity for warm, dense aluminum plasmas and liquids, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.66.025401}{\textit{Phys.~Rev.~E} \textbf{66}, 025401(R)} (2002)

% References on dispersions
\bibitem{bohm-gross_49}
D. Bohm and E.P. Gross, 
Theory of Plasma Oscillations. A. Origin of Medium-Like Behavior,
Phys. Rev. \textbf{75}, 1851 (1949)

\bibitem{bohm-pines-3} D. Bohm, D. Pines, 
{A Collective Description of Electron Interactions: III. Coulomb
 Interactions in a Degenerate Electron Gas}, Phys. Rev. \textbf{92}, 609 (1952)

\bibitem{ferrell-57} R.A. Ferrell, 
{Characteristic Energy Loss of Electrons Passing through Metal Foils. II. Dispersion
Relation and Short Wavelength Cutoff for Plasma Oscillations},
Phys. Rev. \textbf{107}, 450 (1957)

\bibitem{thiele_pre_08} R. Thiele, T. Bornath, C. Fortmann, A. Höll, R. Redmer, H. Reinholz, G. Röpke, A. Wierling,
S. H. Glenzer, and G. Gregori,
Plasmon resonance in warm dense matter,
Phys. Rev. E \textbf{78}, 026411 (2008)

\bibitem{arista-brandt} N.R. Arista and W. Brandt, Dielectric response of quantum plasmas in thermal equilibrium, 
Phys. Rev. A \textbf{29}, 1471 (1984)

\bibitem{dandrea86} R.G. Dandrea, N. Ashcroft, and A.E. Carlsson, Electron liquid at any degeneracy, 
Phys. Rev. B \textbf{34}, 2097 (1986)

\bibitem{glenzer_rmp_09} S. Glenzer and R. Redmer, {X-ray Thomson scattering in high energy density plasmas},
Rev. of Mod. Phys. \textbf{81}, 1625 (2009)

\bibitem{bonitz_pop_94} M. Bonitz, Impossibility of Plasma Instabilities in Isotropic Quantum Plasmas, Phys. Plasmas \textbf{1}, 832 (1994)

\bibitem{bonitz_prl_93} M. Bonitz, R. Binder, and S.W. Koch, Carrier-Acoustic Plasmon Instability in Semiconductor Quantum Wires, Phys. Rev. Lett. \textbf{70}, 3788 (1993)

\bibitem{bonitz_pre_94} M. Bonitz, R. Binder, D.C. Scott, S.W. Koch,  and D. Kremp, Phys. Rev. E \textbf{49}, 5535 (1994)

\bibitem{vladimirov} S.V. Vladimirov and Y.O. Tyshetskiy, On description of a collisionless quantum plasma, Physics
Uspekhi \textbf{54}(12), 1243 (2011)


\bibitem{schakel} A.M.~Schakel, Ground state of electron gases at negative compressibility, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.64.245101}{\textit{Phys.~Rev.~B} \textbf{64}, 245101} (2001)

%%%%%%%%%%%
\end{thebibliography}

